Small-Error Cascaded Group Testing

Group testing concerns itself with the accurate recovery of a set of "defective" items from a larger population via a series of tests. While most works in this area have considered the classical group testing model, where tests are binary and indicate the presence of at least one defective item in the test, we study the cascaded group testing model. In cascaded group testing, tests admit an ordering, and test outcomes indicate the first defective item in the test under this ordering. Under this model, we establish various achievability bounds for several different recovery criteria using both non-adaptive and adaptive test designs when assuming both unconstrained and constrained test sizes. In the constrained test size setting, we also provide a lower bound showing our achievability result is optimal up to logarithmic factors.

==> macros_letters.tex <==
% BLACKBOARD LETTER
\newcommand{\bA}{\mathbb{A}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\bC}{\mathbb{C}}
\newcommand{\bD}{\mathbb{D}}
\newcommand{\bE}{\mathbb{E}}
\newcommand{\bF}{\mathbb{F}}
\newcommand{\bG}{\mathbb{G}}
\newcommand{\bH}{\mathbb{H}}
\newcommand{\bI}{\mathbb{I}}
\newcommand{\bJ}{\mathbb{J}}
\newcommand{\bK}{\mathbb{K}}
\newcommand{\bL}{\mathbb{L}}
\newcommand{\bM}{\mathbb{M}}
\newcommand{\bN}{\mathbb{N}}
\newcommand{\bO}{\mathbb{O}}
\newcommand{\bP}{\mathbb{P}}
\newcommand{\bQ}{\mathbb{Q}}
\newcommand{\bR}{\mathbb{R}}
\newcommand{\bS}{\mathbb{S}}
\newcommand{\bT}{\mathbb{T}}
\newcommand{\bU}{\mathbb{U}}
\newcommand{\bV}{\mathbb{V}}
\newcommand{\bW}{\mathbb{W}}
\newcommand{\bX}{\mathbb{X}}
\newcommand{\bY}{\mathbb{Y}}
\newcommand{\bZ}{\mathbb{Z}}


% BOLDFACE LOWERCASE

\newcommand{\bfa}{\mathbf{a}}
\newcommand{\bfb}{\mathbf{b}}
\newcommand{\bfc}{\mathbf{c}}
\newcommand{\bfd}{\mathbf{d}}
\newcommand{\bfe}{\mathbf{e}}
\newcommand{\bff}{\mathbf{f}}
\newcommand{\bfg}{\mathbf{g}}
\newcommand{\bfh}{\mathbf{h}}
\newcommand{\bfi}{\mathbf{i}}
\newcommand{\bfj}{\mathbf{j}}
\newcommand{\bfk}{\mathbf{k}}
\newcommand{\bfl}{\mathbf{l}}
\newcommand{\bfm}{\mathbf{m}}
\newcommand{\bfn}{\mathbf{n}}
\newcommand{\bfo}{\mathbf{o}}
\newcommand{\bfp}{\mathbf{p}}
\newcommand{\bfq}{\mathbf{q}}
\newcommand{\bfr}{\mathbf{r}}
\newcommand{\bfs}{\mathbf{s}}
\newcommand{\bft}{\mathbf{t}}
\newcommand{\bfu}{\mathbf{u}}
\newcommand{\bfv}{\mathbf{v}}
\newcommand{\bfw}{\mathbf{w}}
\newcommand{\bfx}{\mathbf{x}}
\newcommand{\bfy}{\mathbf{y}}
\newcommand{\bfz}{\mathbf{z}}

% BOLDFACE CAPITAL
\newcommand{\bfA}{\mathbf{A}}
\newcommand{\bfB}{\mathbf{B}}
\newcommand{\bfC}{\mathbf{C}}
\newcommand{\bfD}{\mathbf{D}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bfF}{\mathbf{F}}
\newcommand{\bfG}{\mathbf{G}}
\newcommand{\bfH}{\mathbf{H}}
\newcommand{\bfI}{\mathbf{I}}
\newcommand{\bfJ}{\mathbf{J}}
\newcommand{\bfK}{\mathbf{K}}
\newcommand{\bfL}{\mathbf{L}}
\newcommand{\bfM}{\mathbf{M}}
\newcommand{\bfN}{\mathbf{N}}
\newcommand{\bfO}{\mathbf{O}}
\newcommand{\bfP}{\mathbf{P}}
\newcommand{\bfQ}{\mathbf{Q}}
\newcommand{\bfR}{\mathbf{R}}
\newcommand{\bfS}{\mathbf{S}}
\newcommand{\bfT}{\mathbf{T}}
\newcommand{\bfU}{\mathbf{U}}
\newcommand{\bfV}{\mathbf{V}}
\newcommand{\bfW}{\mathbf{W}}
\newcommand{\bfX}{\mathbf{X}}
\newcommand{\bfY}{\mathbf{Y}}
\newcommand{\bfZ}{\mathbf{Z}}

% BOLDFACE GREEK LETTERS (LOWER AND UPPER)
\newcommand{\bfalpha}{\boldsymbol{\alpha}}
\newcommand{\bfAlpha}{\boldsymbol{\Alpha}}
\newcommand{\bfbeta}{\boldsymbol{\alpha}}
\newcommand{\bfBeta}{\boldsymbol{\Beta}}
\newcommand{\bfgamma}{\boldsymbol{\gamma}}
\newcommand{\bfGamma}{\boldsymbol{\Gamma}}
\newcommand{\bfdelta}{\boldsymbol{\delta}}
\newcommand{\bfDelta}{\boldsymbol{\Delta}}
\newcommand{\bfepsilon}{\boldsymbol{\epsilon}}
\newcommand{\bfZeta}{\boldsymbol{\Zeta}}
\newcommand{\bfeta}{\boldsymbol{\eta}}
\newcommand{\bftheta}{\boldsymbol{\theta}}
\newcommand{\bfTheta}{\boldsymbol{\Theta}}
\newcommand{\bfiota}{\boldsymbol{\theta}}
\newcommand{\bfkappa}{\boldsymbol{\kappa}}
\newcommand{\bflambda}{\boldsymbol{\lambda}}
\newcommand{\bfLambda}{\boldsymbol{\Lambda}}
\newcommand{\bfmu}{\boldsymbol{\mu}}
\newcommand{\bfnu}{\boldsymbol{\nu}}
\newcommand{\bfxi}{\boldsymbol{\xi}}
\newcommand{\bfXi}{\boldsymbol{\Xi}}
\newcommand{\bfpi}{\boldsymbol{\pi}}
\newcommand{\bfPi}{\boldsymbol{\Pi}}
\newcommand{\bfrho}{\boldsymbol{\rho}}
\newcommand{\bfsigma}{\boldsymbol{\sigma}}
\newcommand{\bfSigma}{\boldsymbol{\Sigma}}
\newcommand{\bfphi}{\boldsymbol{\phi}}
\newcommand{\bfPhi}{\boldsymbol{\Phi}}
\newcommand{\bfchi}{\boldsymbol{\chi}}
\newcommand{\bfChi}{\boldsymbol{\Chi}}
\newcommand{\bfpsi}{\boldsymbol{\psi}}
\newcommand{\bfPsi}{\boldsymbol{\Psi}}
\newcommand{\bfomega}{\boldsymbol{\omega}}
\newcommand{\bfOmega}{\boldsymbol{\Omega}}

% CALLIGRAPHIC CAPITALS
\newcommand{\cA}{{\mathcal A}}
\newcommand{\cB}{{\mathcal B}}
\newcommand{\cC}{{\mathcal C}}
\newcommand{\cD}{{\mathcal D}}
\newcommand{\cE}{{\mathcal E}}
\newcommand{\cF}{{\mathcal F}}
\newcommand{\cG}{{\mathcal G}}
\newcommand{\cH}{{\mathcal H}}
\newcommand{\cI}{{\mathcal I}}
\newcommand{\cJ}{{\mathcal J}}
\newcommand{\cK}{{\mathcal K}}
\newcommand{\cL}{{\mathcal L}}
\newcommand{\cM}{{\mathcal M}}
\newcommand{\cN}{{\mathcal N}}
\newcommand{\cO}{{\mathcal O}}
\newcommand{\cP}{{\mathcal P}}
\newcommand{\cQ}{{\mathcal Q}}
\newcommand{\cR}{{\mathcal R}}
\newcommand{\cS}{{\mathcal S}}
\newcommand{\cT}{{\mathcal T}}
\newcommand{\cU}{{\mathcal U}}
\newcommand{\cV}{{\mathcal V}}
\newcommand{\cW}{{\mathcal W}}
\newcommand{\cX}{{\mathcal X}}
\newcommand{\cY}{{\mathcal Y}}
\newcommand{\cZ}{{\mathcal Z}}


% MATHSCRIPT FONT
\newcommand{\sA}{{\mathscr{A}}}
\newcommand{\sB}{{\mathscr{B}}}
\newcommand{\sC}{{\mathscr{C}}}
\newcommand{\sD}{{\mathscr{D}}}
\newcommand{\sE}{{\mathscr{E}}}
\newcommand{\sF}{{\mathscr{F}}}
\newcommand{\sG}{{\mathscr{G}}}
\newcommand{\sH}{{\mathscr{H}}}
\newcommand{\sI}{{\mathscr{I}}}
\newcommand{\sJ}{{\mathscr{J}}}
\newcommand{\sK}{{\mathscr{K}}}
\newcommand{\sL}{{\mathscr{L}}}
\newcommand{\sM}{{\mathscr{M}}}
\newcommand{\sN}{{\mathscr{N}}}
\newcommand{\sO}{{\mathscr{O}}}
\newcommand{\sP}{{\mathscr{P}}}
\newcommand{\sQ}{{\mathscr{Q}}}
\newcommand{\sR}{{\mathscr{R}}}
\newcommand{\sS}{{\mathscr{S}}}
\newcommand{\sT}{{\mathscr{T}}}
\newcommand{\sU}{{\mathscr{U}}}
\newcommand{\sV}{{\mathscr{V}}}
\newcommand{\sW}{{\mathscr{W}}}
\newcommand{\sX}{{\mathscr{X}}}
\newcommand{\sY}{{\mathscr{Y}}}
\newcommand{\sZ}{{\mathscr{Z}}}

% SANS SERIF LOWERCASE
\newcommand{\sfa}{\mathsf{a}}
\newcommand{\sfb}{\mathsf{b}}
\newcommand{\sfc}{\mathsf{c}}
\newcommand{\sfd}{\mathsf{d}}
\newcommand{\sfe}{\mathsf{e}}
\newcommand{\sff}{\mathsf{f}}
\newcommand{\sfg}{\mathsf{g}}
\newcommand{\sfh}{\mathsf{h}}
\newcommand{\sfi}{\mathsf{i}}
\newcommand{\sfj}{\mathsf{j}}
\newcommand{\sfk}{\mathsf{k}}
\newcommand{\sfl}{\mathsf{l}}
\newcommand{\sfm}{\mathsf{m}}
\newcommand{\sfn}{\mathsf{n}}
\newcommand{\sfo}{\mathsf{o}}
\newcommand{\sfp}{\mathsf{p}}
\newcommand{\sfq}{\mathsf{q}}
\newcommand{\sfr}{\mathsf{r}}
\newcommand{\sfs}{\mathsf{s}}
\newcommand{\sft}{\mathsf{t}}
\newcommand{\sfu}{\mathsf{u}}
\newcommand{\sfv}{\mathsf{v}}
\newcommand{\sfw}{\mathsf{w}}
\newcommand{\sfx}{\mathsf{x}}
\newcommand{\sfy}{\mathsf{y}}
\newcommand{\sfz}{\mathsf{z}}

% SANS SERIF UPPERCASE
\newcommand{\sfA}{{\mathsf{A}}}
\newcommand{\sfB}{{\mathsf{B}}}
\newcommand{\sfC}{{\mathsf{C}}}
\newcommand{\sfD}{{\mathsf{D}}}
\newcommand{\sfE}{{\mathsf{E}}}
\newcommand{\sfF}{{\mathsf{F}}}
\newcommand{\sfG}{{\mathsf{G}}}
\newcommand{\sfH}{{\mathsf{H}}}
\newcommand{\sfI}{{\mathsf{I}}}
\newcommand{\sfJ}{{\mathsf{J}}}
\newcommand{\sfK}{{\mathsf{K}}}
\newcommand{\sfL}{{\mathsf{L}}}
\newcommand{\sfM}{{\mathsf{M}}}
\newcommand{\sfN}{{\mathsf{N}}}
\newcommand{\sfO}{{\mathsf{O}}}
\newcommand{\sfP}{{\mathsf{P}}}
\newcommand{\sfQ}{{\mathsf{Q}}}
\newcommand{\sfR}{{\mathsf{R}}}
\newcommand{\sfS}{{\mathsf{S}}}
\newcommand{\sfT}{{\mathsf{T}}}
\newcommand{\sfU}{{\mathsf{U}}}
\newcommand{\sfV}{{\mathsf{V}}}
\newcommand{\sfW}{{\mathsf{W}}}
\newcommand{\sfX}{{\mathsf{X}}}
\newcommand{\sfY}{{\mathsf{Y}}}
\newcommand{\sfZ}{{\mathsf{Z}}}

% UNDERLINE LOWERCASE
\newcommand{\va}{\underline{a}}
\newcommand{\vb}{\underline{b}}
\newcommand{\vc}{\underline{c}}
\newcommand{\vd}{\underline{d}}
\newcommand{\ve}{\underline{e}}
\newcommand{\vf}{\underline{f}}
\newcommand{\vg}{\underline{g}}
\newcommand{\vh}{\underline{h}}
\newcommand{\vi}{\underline{i}}
\newcommand{\vj}{\underline{j}}
\newcommand{\vk}{\underline{k}}
\newcommand{\vl}{\underline{l}}
\newcommand{\vm}{\underline{m}}
\newcommand{\vn}{\underline{n}}
\newcommand{\vo}{\underline{o}}
\newcommand{\vp}{\underline{p}}
\newcommand{\vq}{\underline{q}}
\newcommand{\vr}{\underline{r}}
\newcommand{\vs}{\underline{s}}
\newcommand{\vt}{\underline{t}}
\newcommand{\vu}{\underline{u}}
\newcommand{\vv}{\underline{v}}
\newcommand{\vw}{\underline{w}}
\newcommand{\vx}{\underline{x}}
\newcommand{\vy}{\underline{y}}
\newcommand{\vz}{\underline{z}}

% UNDERLINE UPPERCASE
\newcommand{\vA}{\underline{A}}
\newcommand{\vB}{\underline{B}}
\newcommand{\vC}{\underline{C}}
\newcommand{\vD}{\underline{D}}
\newcommand{\vE}{\underline{E}}
\newcommand{\vF}{\underline{F}}
\newcommand{\vG}{\underline{G}}
\newcommand{\vH}{\underline{H}}
\newcommand{\vI}{\underline{I}}
\newcommand{\vJ}{\underline{J}}
\newcommand{\vK}{\underline{K}}
\newcommand{\vL}{\underline{L}}
\newcommand{\vM}{\underline{M}}
\newcommand{\vN}{\underline{N}}
\newcommand{\vO}{\underline{O}}
\newcommand{\vP}{\underline{P}}
\newcommand{\vQ}{\underline{Q}}
\newcommand{\vR}{\underline{R}}
\newcommand{\vS}{\underline{S}}
\newcommand{\vT}{\underline{T}}
\newcommand{\vU}{\underline{U}}
\newcommand{\vV}{\underline{V}}
\newcommand{\vW}{\underline{W}}
\newcommand{\vX}{\underline{X}}
\newcommand{\vY}{\underline{Y}}
\newcommand{\vZ}{\underline{Z}}

% UNDERLINE GREEK LOWERCASE
\newcommand{\valpha}{\underline{\alpha}}
\newcommand{\vbeta}{\underline{\beta}}
\newcommand{\vgamma}{\underline{\gamma}}
\newcommand{\vdelta}{\underline{\delta}}
\newcommand{\veps}{\underline{\epsilon}}
\newcommand{\vzeta}{\underline{\zeta}}
\newcommand{\veta}{\underline{\eta}}
\newcommand{\vtheta}{\underline{\theta}}
\newcommand{\viota}{\underline{\iota}}
\newcommand{\vkappa}{\underline{\kappa}}
\newcommand{\vlambda}{\underline{\lambda}}
\newcommand{\vmu}{\underline{\mu}}
\newcommand{\vnu}{\underline{\nu}}
\newcommand{\vxi}{\underline{\xi}}
\newcommand{\vpi}{\underline{\pi}}
\newcommand{\vrho}{\underline{\rho}}
\newcommand{\vsigma}{\underline{\sigma}}
\newcommand{\vtau}{\underline{\tau}}
\newcommand{\vupsilon}{\underline{\upsilon}}
\newcommand{\vphi}{\underline{\phi}}
\newcommand{\vchi}{\underline{\chi}}
\newcommand{\vpsi}{\underline{\psi}}
\newcommand{\vomega}{\underline{\omega}}

% BOLD UNDERLINE LOWERCASE
\newcommand{\vbfa}{{\underline{\mathbf{a}}}}
\newcommand{\vbfb}{{\underline{\mathbf{b}}}}
\newcommand{\vbfc}{{\underline{\mathbf{c}}}}
\newcommand{\vbfd}{{\underline{\mathbf{d}}}}
\newcommand{\vbfe}{{\underline{\mathbf{e}}}}
\newcommand{\vbff}{{\underline{\mathbf{f}}}}
\newcommand{\vbfg}{{\underline{\mathbf{g}}}}
\newcommand{\vbfh}{{\underline{\mathbf{h}}}}
\newcommand{\vbfi}{{\underline{\mathbf{i}}}}
\newcommand{\vbfj}{{\underline{\mathbf{j}}}}
\newcommand{\vbfk}{{\underline{\mathbf{k}}}}
\newcommand{\vbfl}{{\underline{\mathbf{l}}}}
\newcommand{\vbfm}{{\underline{\mathbf{m}}}}
\newcommand{\vbfn}{{\underline{\mathbf{n}}}}
\newcommand{\vbfo}{{\underline{\mathbf{o}}}}
\newcommand{\vbfp}{{\underline{\mathbf{p}}}}
\newcommand{\vbfq}{{\underline{\mathbf{q}}}}
\newcommand{\vbfr}{{\underline{\mathbf{r}}}}
\newcommand{\vbfs}{{\underline{\mathbf{s}}}}
\newcommand{\vbft}{{\underline{\mathbf{t}}}}
\newcommand{\vbfu}{{\underline{\mathbf{u}}}}
\newcommand{\vbfv}{{\underline{\mathbf{v}}}}
\newcommand{\vbfw}{{\underline{\mathbf{w}}}}
\newcommand{\vbfx}{{\underline{\mathbf{x}}}}
\newcommand{\vbfy}{{\underline{\mathbf{y}}}}
\newcommand{\vbfz}{{\underline{\mathbf{z}}}}

% BOLD UNDERLINE UPPERCASE
\newcommand{\vbfA}{{\underline{\mathbf{A}}}}
\newcommand{\vbfB}{{\underline{\mathbf{B}}}}
\newcommand{\vbfC}{{\underline{\mathbf{C}}}}
\newcommand{\vbfD}{{\underline{\mathbf{D}}}}
\newcommand{\vbfE}{{\underline{\mathbf{E}}}}
\newcommand{\vbfF}{{\underline{\mathbf{F}}}}
\newcommand{\vbfG}{{\underline{\mathbf{G}}}}
\newcommand{\vbfH}{{\underline{\mathbf{H}}}}
\newcommand{\vbfI}{{\underline{\mathbf{I}}}}
\newcommand{\vbfJ}{{\underline{\mathbf{J}}}}
\newcommand{\vbfK}{{\underline{\mathbf{K}}}}
\newcommand{\vbfL}{{\underline{\mathbf{L}}}}
\newcommand{\vbfM}{{\underline{\mathbf{M}}}}
\newcommand{\vbfN}{{\underline{\mathbf{N}}}}
\newcommand{\vbfO}{{\underline{\mathbf{O}}}}
\newcommand{\vbfP}{{\underline{\mathbf{P}}}}
\newcommand{\vbfQ}{{\underline{\mathbf{Q}}}}
\newcommand{\vbfR}{{\underline{\mathbf{R}}}}
\newcommand{\vbfS}{{\underline{\mathbf{S}}}}
\newcommand{\vbfT}{{\underline{\mathbf{T}}}}
\newcommand{\vbfU}{{\underline{\mathbf{U}}}}
\newcommand{\vbfV}{{\underline{\mathbf{V}}}}
\newcommand{\vbfW}{{\underline{\mathbf{W}}}}
\newcommand{\vbfX}{{\underline{\mathbf{X}}}}
\newcommand{\vbfY}{{\underline{\mathbf{Y}}}}
\newcommand{\vbfZ}{{\underline{\mathbf{Z}}}}

